Modeling Oceanic Variables with Dynamic Graph Neural Networks

Researchers typically resort to numerical methods to understand and predict ocean dynamics, a key task in mastering environmental phenomena. Such methods may not be suitable in scenarios where the topographic map is complex, knowledge about the underlying processes is incomplete, or the application is time critical. On the other hand, if ocean dynamics are observed, they can be exploited by recent machine learning methods. In this paper we describe a data-driven method to predict environmental variables such as current velocity and sea surface height in the region of Santos-Sao Vicente-Bertioga Estuarine System in the southeastern coast of Brazil. Our model exploits both temporal and spatial inductive biases by joining state-of-the-art sequence models (LSTM and Transformers) and relational models (Graph Neural Networks) in an end-to-end framework that learns both the temporal features and the spatial relationship shared among observation sites. We compare our results with the Santos Operational Forecasting System (SOFS). Experiments show that better results are attained by our model, while maintaining flexibility and little domain knowledge dependency.

==> Section/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\begin{table}[htb]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{*{11}{l}}
            \toprule
                               & \multicolumn{2}{c}{\textbf{Speed (m/s)}} & \multicolumn{2}{c}{\textbf{Direction (degrees)}}                                      \\
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            Inputs             & IoA $\uparrow$                           & RMSE $\downarrow$                                & IoA $\uparrow$ & RMSE $\downarrow$ \\
    
            \midrule
            SOFS               & $0.599$                                  & $0.178$                                          & $0.755$        & $85.18$           \\
            Current            & $0.706$                                  & $0.165$                                          & $0.818$        & $70.25$           \\
            Current+SSH      & $\mathbf{0.726}$                                  & $0.158$                                          & $0.842$        & $65.68$           \\
            Current+SSH+Wind & $0.718$                                  & $0.160$                                          & $\mathbf{0.843}$        & $65.29$           \\
            \bottomrule
        \end{tabular}
    }
    \caption{Average results for 10 random seeds using data from all measuring stations to forecast Praticagem station water current speed and direction.}
    \label{tab:current}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{*{11}{l}}
        \toprule
                      & \multicolumn{2}{c}{\textbf{SSH (m)}}                     \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        Inputs        & IoA $\uparrow$                                  & RMSE $\downarrow$ \\

        \midrule
        SOFS          & $0.935$                                         & $0.133$           \\
        SSH     & $\mathbf{0.940}$                                         & $0.124$           \\
        Current+SSH & $0.939$                                         & $0.123$           \\
        \bottomrule
    \end{tabular}
    \caption{Average results for 10 random seeds using data from all measuring stations to forecast Praticagem station sea surface height.}
    \label{tab:elevation}
\end{table}


\begin{table}[htb]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{*{11}{l}}
            \toprule
                               & \multicolumn{2}{c}{\textbf{Speed (m/s)}} & \multicolumn{2}{c}{\textbf{Direction (degrees)}}                                       \\
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            Scenario           & IoA $\uparrow$                           & RMSE  $\downarrow$                               & IoA $\uparrow$ & RMSE  $\downarrow$ \\
    
            \midrule
            Fully disconnected & $0.1$                                    & $0.1$                                            & $0.1$          & $0.1$              \\
            Fully connected    & $0.1$                                    & $0.1$                                            & $0.1$          & $0.1$              \\
            \bottomrule
        \end{tabular}
    }
    \caption{Average results for 10 random seeds comparing disconnected, locally connected and fully connected graphs.}
    \label{tab:booktabs}
\end{table}

\begin{table}[htb]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{*{11}{l}}
            \toprule
                          & \multicolumn{2}{c}{\textbf{Speed (m/s)}} & \multicolumn{2}{c}{\textbf{Direction (degrees)}}                                            \\
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
                          & \multicolumn{2}{c}{IoA}                  & \multicolumn{2}{c}{IoA}                                                                     \\
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            Inputs        & Transformer                              & LSTM                                             & Transformer             & LSTM           \\

            \midrule
            Current       & $\mathbf{0.734}$                  & $0.706$                                   & $\mathbf{0.841}$ & $0.818$ \\
            Current+SSH & $\mathbf{0.762}$                  & $0.726$                                   & $\mathbf{0.860}$ & $0.842$ \\
            \bottomrule
        \end{tabular}
    }
    \caption{Comparison of results for different time series encoders. In these experiments we used a Transformer, a state-of-the-art sequence model, as our first encoders, and compare its results with the previous ones, where we used an LSTM instead. Given the computational cost of Transformers, we used, for each input experiment, the 5 random seeds that gave the best results using LSTM as encoder, and averaged them. We used the same data as the previous experiments to forecast the speed and direction of the water current at Praticagem station.}
    \label{tab:curr_transformervslstm}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{*{11}{l}}
        \toprule
                      & \multicolumn{2}{c}{\textbf{SSH (m)}}\\
        \cmidrule(lr){2-3}
                      & \multicolumn{2}{c}{IoA}\\
        \cmidrule(lr){2-3}
        Inputs & Transformer & LSTM\\

        \midrule
        SSH & $0.932$ & $0.940$ \\
        Current+SSH & $0.939$ & $0.939$ \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of results for different time series encoders. Same experimental design as showed in \ref{tab:curr_transformervslstm}, except that we used sea surface height as solo input in one experiment, and we forecast the SSH at Praticagem station.}
    \label{tab:elev_transformervslstm}
\end{table}

